Petabytes to Science

A Kavli foundation sponsored workshop on the theme \emph{Petabytes to Science} was held 12$^{th}$ to 14$^{th}$ of February 2019 in Las Vegas. The aim of the this workshop was to discuss important trends and technologies which may support astronomy. We also tackled how to better shape the workforce for the new trends and how we should approach education and public outreach. This document was coauthored during the workshop and edited in the weeks after. It comprises the discussions and highlights many recommendations which came out of the workshop. We shall distill parts of this document and formulate potential white papers for the decadal survey.

==> reclist.tex <==
\protect \unhbox \voidb@x \bgroup \def \linenoprevgraf \prevgraf \def 0{0}\interlinepenalty -\int@parpenalty \def 100{100}\brokenpenalty \@ne \def 10000{10000}\clubpenalty \tw@ \def 10000{10000}\widowpenalty \f@ur \def 50{50}\displaywidowpenalty 8\relax \@@@par \@tempdima \prevdepth \setbox \@tempboxa \hbox {}\dp \@tempboxa =\@tempdima \prevdepth -\@m \p@ \kern -\@tempdima \box \@tempboxa \interlinepenalty 0\brokenpenalty 100\clubpenalty 10000\widowpenalty 10000\displaywidowpenalty 50\relax 

